The Broken Rung: Gender and the Leadership Gap

Addressing female underrepresentation in leadership positions has become a key policy objective. However, little is known about the extent to which leadership appeals differently to women. Collecting new data from a large firm, I document that women are substantially less likely to apply for early-career promotions. Realized application patterns and large-scale surveys reveal the role of an understudied feature of promotions -- having to assume responsibility over a team -- which is less appealing to women. This gender difference is not accounted for by standard explanations, such as success likelihood or confidence, but is rather a product of common design features of leadership positions.

==> Tables/a5_table_copy.tex <==
{
	\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
	\begin{tabular}{l*{5}{c}}
		\hline\hline
  \noalign{\vskip 2mm} 
		\textit{Outcome:}             &\multicolumn{2}{c}{Lower}  &   &\multicolumn{2}{c}{First Leadership} \\ 
     &\multicolumn{2}{c}{Level}  &   &\multicolumn{2}{c}{Level} \\\cline{2-3}  \cline{5-6}  
\noalign{\vskip 2mm}
&\multicolumn{1}{c}{Entry}&\multicolumn{1}{c}{Exit}&&\multicolumn{1}{c}{Entry}&\multicolumn{1}{c}{(Exit}\\
		&\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
		\hline
   Female  &      -0.108\sym{**} &-0.176\sym{***}&  &       0.188         &          -0.239         \\
&     (0.044)               &     (0.060)         & &     (0.205)  &     (0.216)         \\
\hline
Outcome Mean        &      0.0138              &      0.0067         &&      0.0040    &      0.0051         \\
Av ME for Women     &     -0.0039        &     -0.0013         & &      0.0072         &     -0.0011         \\
Gender Gap in \%    &       -28.0         &       -19.8         &  &       177.9        &     -21.5         \\
Observations   &        3xx,xxx              &           3xx,xxx         &   &          6x,xxx    &         6x,xxx               \\
\hline\hline \multicolumn{6}{p{0.7\linewidth}}{\footnotesize \textit{Notes}:  This table documents gender differences in the likelihood of entry to and exit from the firm in a given quarter. Columns 1 and 2 focus on employees in lower-level positions who work as individual contributors without enhanced job responsibility (hierarchy ranking of 20 or below). Columns 3 and 4 focus on employees in first-level leadership positions, for instance those who lead a team, head a project, or work as an expert with enhanced job responsibility (hierarchy ranking between 20 and 40). Each coefficient stems from a separate logit regression of an indicator for entry or exit on gender and a large set of controls. Gender gaps in \% are computed by dividing the average marginal effect for women based on the logit coefficient by the outcome mean. Controls: Age, German citizenship, educational qualification, marital status, family status, parental leave, firm tenure,  function, division,  location, full-time, hours, number of direct reports, and quarter fixed effects. Standard errors in parentheses. *p$<$ 0.10, **p$<$ 0.05, ***p$<$ 0.001} \\ \end{tabular}}




==> Tables/raw/1_table.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{ccc}}
\hline\hline
                    &\multicolumn{3}{c}{none}              \\
                    &         Men&       Women&      p-vaue\\
\hline
German citizen      &        0.89&        0.84&        0.00\\
Age (years)         &        43.9&        40.2&        0.00\\
Education (years)   &        16.0&        14.9&        0.00\\
Firm tenure (years) &        13.3&        11.9&        0.00\\
Married             &        0.64&        0.50&        0.00\\
Children            &        0.77&        0.64&        0.00\\
On parental leave   &        0.02&        0.08&        0.00\\
Full-time           &        0.98&        0.74&        0.00\\
Weekly hours        &        42.2&        37.9&        0.00\\
Technical position  &        0.72&        0.34&        0.00\\
Salary decile       &         6.0&         3.5&        0.00\\
Top management      &        0.08&        0.04&        0.00\\
Team leadership     &        0.21&        0.09&        0.00\\
Direct reports      &         6.1&         5.1&        0.00\\
Cumulative reports  &        37.0&        10.7&        0.00\\
\hline
Observations        &      440151&            &            \\
\hline\hline
\multicolumn{4}{l}{\footnotesize }\\
\end{tabular}
}


==> Tables/raw/2_table.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{1}{c}{Reports}&\multicolumn{1}{c}{Autonomy}&\multicolumn{1}{c}{Reporting}&\multicolumn{1}{c}{PCA}&\multicolumn{1}{c}{PCA+Pay}&\multicolumn{1}{c}{Pay}\\
\hline
main                &                     &                     &                     &                     &                     &                     \\
Female              &      -0.357\sym{***}&      -0.131\sym{***}&       0.041         &      -0.297\sym{***}&      -0.251\sym{***}&      -0.141\sym{**} \\
                    &     (0.061)         &     (0.035)         &     (0.048)         &     (0.071)         &     (0.084)         &     (0.065)         \\
\hline
Outcome Mean        &      0.0079         &      0.0181         &      0.0093         &      0.0055         &      0.0038         &      0.0052         \\
Av ME for Women     &     -0.0024         &     -0.0028         &      0.0004         &     -0.0015         &     -0.0009         &     -0.0009         \\
Gender Gap in \%    &       -30.2         &       -15.4         &         4.7         &       -27.4         &       -24.4         &       -17.8         \\
Observations        &      358790         &      358790         &      358790         &      358790         &      358790         &      339349         \\
\hline\hline \multicolumn{7}{p{\linewidth}}{\footnotesize \textit{Notes}: Standard errors in parentheses. *p$<$ 0.10, **p$<$ 0.05, ***p$<$ 0.001.}\\ \end{tabular}}


==> Tables/raw/3_table.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
                    &\multicolumn{1}{c}{Lower-Level}&\multicolumn{1}{c}{First Leadership Level}&\multicolumn{1}{c}{Any Leadership Level}\\
\hline
Applied for promotion&                     &                     &                     \\
Female              &      -0.297\sym{***}&       0.005         &      -0.036         \\
                    &     (0.071)         &     (0.170)         &     (0.169)         \\
\hline
Outcome Mean        &      0.0055         &      0.0048         &      0.0041         \\
Av ME for Women     &     -0.0015         &      0.0000         &     -0.0002         \\
Gender Gap in \%    &       -27.4         &         0.8         &        -5.2         \\
Observations        &      358790         &       60615         &       71987         \\
\hline\hline \multicolumn{4}{p{\linewidth}}{\footnotesize \textit{Notes}: Standard errors in parentheses. *p$<$ 0.10, **p$<$ 0.05, ***p$<$ 0.001.}\\ \end{tabular}}


==> Tables/raw/3_table_autonomy.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
                    &\multicolumn{1}{c}{Lower-Level}&\multicolumn{1}{c}{First Leadership Level}&\multicolumn{1}{c}{Any Leadership Level}\\
\hline
applied\_more\_autonomy&                     &                     &                     \\
Female              &      -0.131\sym{***}&       0.155         &       0.104         \\
                    &     (0.035)         &     (0.134)         &     (0.133)         \\
\hline
Outcome Mean        &      0.0181         &      0.0100         &      0.0085         \\
Av ME for Women     &     -0.0028         &      0.0018         &      0.0011         \\
Gender Gap in \%    &       -15.4         &        18.4         &        12.8         \\
Observations        &      358790         &       60615         &       71987         \\
\hline\hline \multicolumn{4}{p{\linewidth}}{\footnotesize \textit{Notes}: Standard errors in parentheses. *p$<$ 0.10, **p$<$ 0.05, ***p$<$ 0.001.}\\ \end{tabular}}


==> Tables/raw/3_table_distance.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
                    &\multicolumn{1}{c}{Lower-Level}&\multicolumn{1}{c}{First Leadership Level}&\multicolumn{1}{c}{Any Leadership Level}\\
\hline
applied\_closer\_report&                     &                     &                     \\
Female              &       0.041         &      -0.104         &      -0.076         \\
                    &     (0.048)         &     (0.189)         &     (0.180)         \\
\hline
Outcome Mean        &      0.0093         &      0.0065         &      0.0058         \\
Av ME for Women     &      0.0004         &     -0.0007         &     -0.0005         \\
Gender Gap in \%    &         4.7         &       -11.0         &        -8.3         \\
Observations        &      358790         &       56209         &       66896         \\
\hline\hline \multicolumn{4}{p{\linewidth}}{\footnotesize \textit{Notes}: Standard errors in parentheses. *p$<$ 0.10, **p$<$ 0.05, ***p$<$ 0.001.}\\ \end{tabular}}


==> Tables/raw/3_table_pay.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
                    &\multicolumn{1}{c}{Lower-Level}&\multicolumn{1}{c}{First Leadership Level}&\multicolumn{1}{c}{Any Leadership Level}\\
\hline
applied\_muchmore\_earnings&                     &                     &                     \\
Female              &      -0.141\sym{**} &       0.363\sym{**} &       0.402\sym{**} \\
                    &     (0.065)         &     (0.184)         &     (0.180)         \\
\hline
Outcome Mean        &      0.0052         &      0.0048         &      0.0042         \\
Av ME for Women     &     -0.0009         &      0.0023         &      0.0024         \\
Gender Gap in \%    &       -17.8         &        48.9         &        56.2         \\
Observations        &      339349         &       56951         &       67669         \\
\hline\hline \multicolumn{4}{p{\linewidth}}{\footnotesize \textit{Notes}: Standard errors in parentheses. *p$<$ 0.10, **p$<$ 0.05, ***p$<$ 0.001.}\\ \end{tabular}}


==> Tables/raw/3_table_reports.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
                    &\multicolumn{1}{c}{Lower-Level}&\multicolumn{1}{c}{First Leadership Level}&\multicolumn{1}{c}{Any Leadership Level}\\
\hline
applied\_leader\_more &                     &                     &                     \\
Female              &      -0.357\sym{***}&      -0.072         &      -0.117         \\
                    &     (0.061)         &     (0.133)         &     (0.133)         \\
\hline
Outcome Mean        &      0.0079         &      0.0107         &      0.0092         \\
Av ME for Women     &     -0.0024         &     -0.0009         &     -0.0013         \\
Gender Gap in \%    &       -30.2         &        -8.5         &       -14.3         \\
Observations        &      358790         &       60615         &       71987         \\
\hline\hline \multicolumn{4}{p{\linewidth}}{\footnotesize \textit{Notes}: Standard errors in parentheses. *p$<$ 0.10, **p$<$ 0.05, ***p$<$ 0.001.}\\ \end{tabular}}


==> Tables/raw/4_table.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{1}{c}{Lateral Switch}&\multicolumn{1}{c}{Different Function}&\multicolumn{1}{c}{Different Division}&\multicolumn{1}{c}{Different Location}&\multicolumn{1}{c}{Promotion Same location}&\multicolumn{1}{c}{Promotion Different location}\\
\hline
main                &                     &                     &                     &                     &                     &                     \\
Female              &       0.132\sym{**} &       0.117         &       0.221\sym{***}&       0.139         &      -0.316\sym{***}&      -0.246\sym{*}  \\
                    &     (0.057)         &     (0.085)         &     (0.081)         &     (0.106)         &     (0.086)         &     (0.128)         \\
\hline
Outcome Mean        &      0.0065         &      0.0027         &      0.0029         &      0.0020         &      0.0038         &      0.0018         \\
Av ME for Women     &      0.0009         &      0.0004         &      0.0008         &      0.0003         &     -0.0011         &     -0.0004         \\
Gender Gap in \%    &        14.4         &        15.4         &        26.9         &        14.7         &       -30.1         &       -21.3         \\
Observations        &      358790         &      358790         &      358790         &      358790         &      358790         &      358790         \\
\hline\hline \multicolumn{7}{p{\linewidth}}{\footnotesize \textit{Notes}: Standard errors in parentheses. *p$<$ 0.10, **p$<$ 0.05, ***p$<$ 0.001.}\\ \end{tabular}}


==> Tables/raw/5_table.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{1}{c}{Works Full-time}&\multicolumn{1}{c}{No Children}&\multicolumn{1}{c}{Not Married}&\multicolumn{1}{c}{Female-Leaning Function}&\multicolumn{1}{c}{Female Manager}&\multicolumn{1}{c}{High-Female Team}\\
\hline
Applied for promotion&                     &                     &                     &                     &                     &                     \\
Female              &      -0.322\sym{***}&      -0.216\sym{**} &      -0.244\sym{**} &      -0.704\sym{***}&      -0.519\sym{***}&      -0.345\sym{***}\\
                    &     (0.073)         &     (0.105)         &     (0.097)         &     (0.117)         &     (0.164)         &     (0.080)         \\
\hline
Outcome Mean        &      0.0058         &      0.0060         &      0.0057         &      0.0057         &      0.0069         &      0.0058         \\
Av ME for Women     &     -0.0020         &     -0.0013         &     -0.0013         &     -0.0037         &     -0.0031         &     -0.0018         \\
Gender Gap in \%    &       -34.0         &       -22.0         &       -23.6         &       -65.2         &       -44.8         &       -31.5         \\
Observations        &      331455         &      103607         &      151814         &       80529         &       33190         &      166522         \\
\hline\hline \multicolumn{7}{p{\linewidth}}{\footnotesize \textit{Notes}: Standard errors in parentheses. *p$<$ 0.10, **p$<$ 0.05, ***p$<$ 0.001.}\\ \end{tabular}}


==> Tables/raw/6_table.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{7}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}&\multicolumn{1}{c}{(7)}\\
                    &\multicolumn{1}{c}{\shortstack{Full-time}}&\multicolumn{1}{c}{\shortstack{No Children}}&\multicolumn{1}{c}{\shortstack{Female-Leaning\\Function}}&\multicolumn{1}{c}{\shortstack{High Risk}}&\multicolumn{1}{c}{\shortstack{High Competition}}&\multicolumn{1}{c}{\shortstack{High\\Confidence}}&\multicolumn{1}{c}{\shortstack{Effective\\Leader}}\\
                    &aspiration\_team         &aspiration\_team         &aspiration\_team         &aspiration\_team         &aspiration\_team         &aspiration\_team         &aspiration\_team         \\
\hline
Female              &      -0.396\sym{***}&      -0.428\sym{***}&      -0.473\sym{***}&      -0.468\sym{***}&      -0.465\sym{***}&      -0.437\sym{***}&      -0.436\sym{***}\\
                    &    (0.0943)         &    (0.1167)         &    (0.1405)         &    (0.1305)         &    (0.1049)         &    (0.0985)         &    (0.0900)         \\
\hline
Outcome mean        &       0.249         &       0.228         &       0.254         &       0.281         &       0.287         &       0.241         &       0.286         \\
Female Coefficient  &      -0.072         &      -0.075         &      -0.081         &      -0.089         &      -0.089         &      -0.073         &      -0.084         \\
Gender Gap in \%    &       -29.1         &       -32.8         &       -32.0         &       -31.8         &       -31.0         &       -30.4         &       -29.4         \\
Observations        &    4533.000         &    2542.000         &    1410.000         &    2186.000         &    3256.000         &    4351.000         &    4383.000         \\
\hline\hline
\multicolumn{8}{l}{\footnotesize Controls: Age, tenure, children,  full-time, hours, division, functional area}\\
\multicolumn{8}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Tables/raw/a1_table.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
                    &\multicolumn{1}{c}{\shortstack{Analysis sample}}&\multicolumn{1}{c}{\shortstack{Large manufacturer}}&\multicolumn{1}{c}{\shortstack{German workforce}}\\
\hline
female              &        0.21&        0.21&        0.45\\
German citizen      &        0.88&        0.85&        0.88\\
Age (years)         &        43.1&        44.1&        43.9\\
Married             &        0.61&        0.59&        0.54\\
Children            &        0.80&        0.62&        0.62\\
Education (years)   &        15.7&        11.7&        11.8\\
Firm tenure (years) &        13.1&        16.8&        13.2\\
Weekly hours        &        41.2&        40.5&        38.1\\
Team leadership     &        0.18&        0.25&        0.29\\
\hline
Observations        &       93505&        1472&       13791\\
\hline\hline \multicolumn{4}{p{1.1\linewidth}}{\footnotesize Notes: This Table reports average characteristics for 2018. Column 1 reports statistics for my main analysis sample. Column 2 uses data from the BiBB survey on white-collar employees at manufacturing firms with at least 100 employees in West Germany. Column 3 uses data from the BiBB survey for all labor force participants in West Germany. Column 2 and 3 are weighted to achive representativeness of the German population.}\\ \end{tabular}}


==> Tables/raw/a2_table.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{1}{c}{Reports}&\multicolumn{1}{c}{Autonomy}&\multicolumn{1}{c}{Distance}&\multicolumn{1}{c}{Pay}&\multicolumn{1}{c}{Combined}&\multicolumn{1}{c}{Combined}\\
\hline
main                &                     &                     &                     &                     &                     &                     \\
Female              &      -0.354\sym{***}&      -0.136\sym{***}&       0.040         &      -0.219\sym{**} &      -0.232\sym{***}&      -0.278\sym{***}\\
                    &     (0.058)         &     (0.035)         &     (0.068)         &     (0.110)         &     (0.080)         &     (0.066)         \\
\hline
Outcome Mean        &      0.0088         &      0.0205         &      0.0114         &      0.0048         &      0.0055         &      0.0057         \\
Av ME for Women     &     -0.0026         &     -0.0031         &      0.0006         &     -0.0011         &     -0.0011         &     -0.0015         \\
Gender Gap in \%    &       -30.0         &       -15.1         &         5.0         &       -23.9         &       -20.8         &       -26.6         \\
Pseudo R-squared    &      351147         &      300358         &      169339         &      101541         &      276457         &      398676         \\
\hline\hline \multicolumn{7}{p{\linewidth}}{\footnotesize \textit{Notes}: Standard errors in parentheses. *p$<$ 0.10, **p$<$ 0.05, ***p$<$ 0.001.}\\ \end{tabular}}


==> Tables/raw/a2_table_panela.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                    &\multicolumn{1}{c}{Demo}&\multicolumn{1}{c}{Position}&\multicolumn{1}{c}{Performance}&\multicolumn{1}{c}{Time in position}\\
\hline
Applied for promotion&                     &                     &                     &                     \\
Female              &      -0.351\sym{***}&      -0.389\sym{***}&      -0.214\sym{***}&      -0.298\sym{***}\\
                    &     (0.062)         &     (0.066)         &     (0.073)         &     (0.071)         \\
\hline
Outcome Mean        &      0.0055         &      0.0055         &      0.0055         &      0.0055         \\
Av ME for Women     &     -0.0018         &     -0.0021         &     -0.0013         &     -0.0015         \\
Gender Gap in \%    &       -33.3         &       -37.1         &       -22.8         &       -27.4         \\
Observations        &      359608         &      367413         &      303580         &      358790         \\
\hline\hline \multicolumn{5}{p{\linewidth}}{\footnotesize \textit{Notes}: Standard errors in parentheses. *p$<$ 0.10, **p$<$ 0.05, ***p$<$ 0.001.}\\ \end{tabular}}


==> Tables/raw/a2_table_panelb.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
                    &\multicolumn{1}{c}{Balanced}&\multicolumn{1}{c}{Conditional}&\multicolumn{1}{c}{Rejected in Past}\\
\hline
Applied for promotion&                     &                     &                     \\
Female              &      -0.283\sym{***}&      -0.277\sym{***}&      -0.352\sym{***}\\
                    &     (0.082)         &     (0.076)         &     (0.120)         \\
\hline
Outcome Mean        &      0.0056         &      0.1928         &      0.0333         \\
Av ME for Women     &     -0.0014         &     -0.0345         &     -0.0087         \\
Gender Gap in \%    &       -25.6         &       -17.9         &       -26.2         \\
Observations        &      289885         &       10507         &       23661         \\
\hline\hline \multicolumn{4}{p{\linewidth}}{\footnotesize \textit{Notes}: Standard errors in parentheses. *p$<$ 0.10, **p$<$ 0.05, ***p$<$ 0.001.}\\ \end{tabular}}


==> Tables/raw/a3_table.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
                    &\multicolumn{1}{c}{Interview Promotion}&\multicolumn{1}{c}{Hired Promotion}\\
\hline
main                &                     &                     \\
Female              &       0.568\sym{***}&       0.525\sym{***}\\
                    &     (0.138)         &     (0.176)         \\
\hline
Outcome Mean        &      0.5479         &      0.1553         \\
Av ME for Women     &      0.1283         &      0.0700         \\
Gender Gap in \%    &        23.4         &        45.1         \\
LR chi2             &        2029         &        2029         \\
\hline\hline \multicolumn{3}{p{\linewidth}}{\footnotesize \textit{Notes}: Standard errors in parentheses. *p$<$ 0.10, **p$<$ 0.05, ***p$<$ 0.001.}\\ \end{tabular}}


==> Tables/raw/a3_table_panela.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                    &\multicolumn{1}{c}{Demo}&\multicolumn{1}{c}{Position}&\multicolumn{1}{c}{Performance}&\multicolumn{1}{c}{Time in position}\\
\hline
Applied for promotion&                     &                     &                     &                     \\
Female              &      -0.351\sym{***}&      -0.389\sym{***}&      -0.214\sym{***}&      -0.298\sym{***}\\
                    &     (0.062)         &     (0.066)         &     (0.073)         &     (0.071)         \\
\hline
Outcome Mean        &      0.0055         &      0.0055         &      0.0055         &      0.0055         \\
Av ME for Women     &     -0.0018         &     -0.0021         &     -0.0013         &     -0.0015         \\
Gender Gap in \%    &       -33.3         &       -37.1         &       -22.8         &       -27.4         \\
Observations        &      359608         &      367413         &      303580         &      358790         \\
\hline\hline \multicolumn{5}{p{\linewidth}}{\footnotesize \textit{Notes}: Standard errors in parentheses. *p$<$ 0.10, **p$<$ 0.05, ***p$<$ 0.001.}\\ \end{tabular}}


==> Tables/raw/a3_table_panelb.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
                    &\multicolumn{1}{c}{Balanced}&\multicolumn{1}{c}{Conditional}&\multicolumn{1}{c}{Rejected in Past}\\
\hline
Applied for promotion&                     &                     &                     \\
Female              &      -0.283\sym{***}&      -0.277\sym{***}&      -0.352\sym{***}\\
                    &     (0.082)         &     (0.076)         &     (0.120)         \\
\hline
Outcome Mean        &      0.0056         &      0.1928         &      0.0333         \\
Av ME for Women     &     -0.0014         &     -0.0345         &     -0.0087         \\
Gender Gap in \%    &       -25.6         &       -17.9         &       -26.2         \\
Observations        &      289885         &       10507         &       23661         \\
\hline\hline \multicolumn{4}{p{\linewidth}}{\footnotesize \textit{Notes}: Standard errors in parentheses. *p$<$ 0.10, **p$<$ 0.05, ***p$<$ 0.001.}\\ \end{tabular}}


==> Tables/raw/a4_table.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
                    &\multicolumn{1}{c}{Interview Promotion}&\multicolumn{1}{c}{Hired Promotion}\\
\hline
main                &                     &                     \\
Female              &       0.568\sym{***}&       0.525\sym{***}\\
                    &     (0.138)         &     (0.176)         \\
\hline
Outcome Mean        &      0.5479         &      0.1553         \\
Av ME for Women     &      0.1283         &      0.0700         \\
Gender Gap in \%    &        23.4         &        45.1         \\
LR chi2             &        2029         &        2029         \\
\hline\hline \multicolumn{3}{p{\linewidth}}{\footnotesize \textit{Notes}: Standard errors in parentheses. *p$<$ 0.10, **p$<$ 0.05, ***p$<$ 0.001.}\\ \end{tabular}}


==> Tables/raw/a5_table.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                    &\multicolumn{1}{c}{Lower-Level}&\multicolumn{1}{c}{First Leadership Level}&\multicolumn{1}{c}{Lower-Level}&\multicolumn{1}{c}{First Leadership Level}\\
\hline
main                &                     &                     &                     &                     \\
Female              &      -0.108\sym{**} &       0.188         &      -0.176\sym{***}&      -0.239         \\
                    &     (0.044)         &     (0.205)         &     (0.060)         &     (0.216)         \\
\hline
Outcome Mean        &      0.0138         &      0.0040         &      0.0067         &      0.0051         \\
Av ME for Women     &     -0.0039         &      0.0072         &     -0.0013         &     -0.0011         \\
Gender Gap in \%    &       -28.0         &       177.9         &       -19.8         &       -21.5         \\
Observations        &      110152         &        6088         &      358790         &       60615         \\
\hline\hline \multicolumn{5}{p{\linewidth}}{\footnotesize \textit{Notes}: Standard errors in parentheses. *p$<$ 0.10, **p$<$ 0.05, ***p$<$ 0.001.}\\ \end{tabular}}


==> Tables/raw/a6_table.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{1}{c}{X}&\multicolumn{1}{c}{Risk}&\multicolumn{1}{c}{Competition}&\multicolumn{1}{c}{General confidence}&\multicolumn{1}{c}{Admin + conflict}&\multicolumn{1}{c}{Overtime}\\
\hline
Q3: Applied for leadership in past 12 mos&                     &                     &                     &                     &                     &                     \\
Female              &      -0.430\sym{***}&      -0.329\sym{*}  &      -0.378\sym{**} &      -0.387\sym{**} &      -0.255\sym{*}  &      -0.232\sym{*}  \\
                    &     (0.137)         &     (0.183)         &     (0.154)         &     (0.152)         &     (0.138)         &     (0.138)         \\
\hline
Outcome Mean        &      0.0817         &      0.1255         &      0.1214         &      0.0941         &      0.0817         &      0.0817         \\
Av ME for Women     &     -0.0277         &     -0.0341         &     -0.0354         &     -0.0288         &     -0.0149         &     -0.0134         \\
Gender Gap in \%    &       -33.9         &       -27.2         &       -29.2         &       -30.6         &       -18.2         &       -16.4         \\
Pseudo R-squared    &        6020         &        2188         &        3262         &        4369         &        5890         &        5878         \\
\hline\hline \multicolumn{7}{p{\linewidth}}{\footnotesize \textit{Notes}: Standard errors in parentheses. *p$<$ 0.10, **p$<$ 0.05, ***p$<$ 0.001.}\\ \end{tabular}}


==> Tables/raw/b1_table.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
                    &\multicolumn{1}{c}{Interview Promotion}&\multicolumn{1}{c}{Hired Promotion}\\
\hline
main                &                     &                     \\
Female              &       1.501\sym{***}&       1.425\sym{*}  \\
                    &     (0.541)         &     (0.772)         \\
\hline
Outcome Mean        &      0.4815         &      0.1650         \\
Av ME for Women     &      0.2722         &      0.1758         \\
Gender Gap in \%    &        56.5         &       106.5         \\
LR chi2             &         297         &         232         \\
\hline\hline \multicolumn{3}{p{\linewidth}}{\footnotesize \textit{Notes}: Standard errors in parentheses. *p$<$ 0.10, **p$<$ 0.05, ***p$<$ 0.001.}\\ \end{tabular}}


==> Tables/raw/b2_table.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{1}{c}{Career Planning}&\multicolumn{1}{c}{Interest Applying}&\multicolumn{1}{c}{Applied}&\multicolumn{1}{c}{Career Planning}&\multicolumn{1}{c}{Interest Applying}&\multicolumn{1}{c}{Applied}\\
\hline
main                &                     &                     &                     &                     &                     &                     \\
Female              &      -0.575\sym{***}&      -0.739\sym{***}&      -0.542\sym{*}  &      -0.575\sym{***}&      -0.739\sym{***}&      -0.542\sym{*}  \\
                    &     (0.222)         &     (0.192)         &     (0.284)         &     (0.222)         &     (0.192)         &     (0.284)         \\
race\_minority=1     &       0.196         &       0.189         &       0.463\sym{**} &       0.196         &       0.189         &       0.463\sym{**} \\
                    &     (0.177)         &     (0.155)         &     (0.226)         &     (0.177)         &     (0.155)         &     (0.226)         \\
\hline
Outcome Mean        &      0.2287         &      0.3512         &      0.1232         &      0.2287         &      0.3512         &      0.1232         \\
Av ME for Women     &     -0.0888         &     -0.1478         &     -0.0479         &      0.0337         &      0.0400         &      0.0524         \\
Gender Gap in \%    &       -38.8         &       -42.1         &       -38.9         &        14.7         &        11.4         &        42.5         \\
Observations        &         922         &         924         &         926         &         922         &         924         &         926         \\
\hline\hline \multicolumn{7}{p{\linewidth}}{\footnotesize \textit{Notes}: Standard errors in parentheses. *p$<$ 0.10, **p$<$ 0.05, ***p$<$ 0.001.}\\ \end{tabular}}


==> Tables/raw/c3_table.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}\\
                    &\multicolumn{1}{c}{Sample}&\multicolumn{1}{c}{Survey 1}&\multicolumn{1}{c}{Survey 2}\\
\hline
Age $<$30           &        0.10&        0.11&        0.07\\
Age 30-39           &        0.31&        0.27&        0.25\\
Age 40-49           &        0.30&        0.22&        0.24\\
Age $>=$50          &        0.29&        0.24&        0.26\\
Tenure $<=$ 2       &        0.10&        0.12&        0.04\\
Tenure 3-5          &        0.12&        0.15&        0.12\\
Tenure 6-9          &        0.13&        0.15&        0.15\\
Tenure $>=$10       &        0.55&        0.44&        0.51\\
Any children        &        0.74&        0.58&        0.63\\
Weekly hours        &       41.30&       40.47&       40.39\\
Engineering         &        0.49&        0.36&        0.31\\
Finance & Law       &        0.08&        0.05&        0.05\\
HR                  &        0.03&        0.03&        0.04\\
IT                  &        0.05&        0.04&        0.05\\
Marketing and Sales &        0.10&        0.06&        0.06\\
Logistics           &        0.05&        0.04&        0.04\\
Purchasing          &        0.04&        0.03&        0.03\\
Quality             &        0.07&        0.07&        0.06\\
\hline
Observations        &      440151&       16652&       12065\\
\hline\hline
\multicolumn{4}{l}{\footnotesize }\\
\end{tabular}
}


==> Tables/raw/c4_table.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         \\
                    &completed\_before1reminder         &completed\_before1reminder         \\
\hline
Female              &       0.057         &      -0.034         \\
                    &    (0.0481)         &    (0.0550)         \\
\hline
Outcome mean        &       0.616         &       0.550         \\
Av ME for Women     &       0.013         &      -0.008         \\
Gender Gap in \%    &         2.0         &        -1.5         \\
Adj R-Squared       &       0.014         &       0.004         \\
Observations        &       13808         &        9186         \\
\hline\hline
\multicolumn{3}{l}{\footnotesize Controls: age, tenure, children, hours, functional area}\\
\multicolumn{3}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> Tables/raw/hierarchy_1_table.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{cccc}}
\hline\hline
                    &\multicolumn{4}{c}{(1)}                            \\
                    &\multicolumn{4}{c}{}                               \\
                    &Share external hire&Tenure (years)&Share $>=$ BA degree&Share bonus/pay\\
\hline
0-10                &       0.015&        11.6&        0.41&        0.12\\
10-20               &       0.011&        13.4&        0.54&        0.13\\
20-30               &       0.005&        16.2&        0.72&        0.16\\
30-40               &       0.002&        17.4&        0.78&        0.22\\
40-50               &       0.001&        17.3&        0.78&        0.30\\
50-60               &       0.000&        16.8&        0.79&        0.40\\
60-100              &       0.001&        16.1&        0.75&        0.40\\
Total               &       0.012&        13.0&        0.51&        0.14\\
\hline
Observations        &      440151&            &            &            \\
\hline\hline
\multicolumn{5}{l}{\footnotesize }\\
\end{tabular}
}


==> Tables/raw/hierarchy_2_table.tex <==
 & \multicolumn{7}{c}{lead1yr\_hierarchy} \\
hierarchy&1&2&3&4&5&6&Total \\
&\%&\%&\%&\%&\%&\%&\% \\
\midrule
0-10&68.5&27.4&3.4&0.6&0.0&0.0&100.0 \\
10-20&20.1&58.6&17.8&2.7&0.7&0.0&100.0 \\
20-30&0.5&17.3&50.0&26.8&5.5&0.0&100.0 \\
30-40&0.0&5.8&32.6&45.3&15.1&1.2&100.0 \\
40-50&0.0&0.0&17.9&35.7&35.7&10.7&100.0 \\
50-60&0.0&0.0&25.0&25.0&25.0&25.0&100.0 \\
Total&41.1&35.3&14.7&6.6&2.0&0.2&100.0 \\
\midrule
N&832&713&298&133&41&5&2,022 \\


==> Tables/top_4_table.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{6}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}&\multicolumn{1}{c}{(5)}&\multicolumn{1}{c}{(6)}\\
                    &\multicolumn{1}{c}{Lateral Switch}&\multicolumn{1}{c}{Different Function}&\multicolumn{1}{c}{Different Division}&\multicolumn{1}{c}{Different Location}&\multicolumn{1}{c}{Promotion Same location}&\multicolumn{1}{c}{Promotion Different location}\\
\hline
main                &                     &                     &                     &                     &                     &                     \\
Female              &      -0.106         &       0.031         &       0.004         &      -0.109         &      -0.002         &      -0.142         \\
                    &     (0.125)         &     (0.097)         &     (0.102)         &     (0.134)         &     (0.199)         &     (0.334)         \\
\hline
Outcome Mean        &      0.0132         &      0.0191         &      0.0172         &      0.0122         &      0.0030         &      0.0018         \\
Av ME for Women     &     -0.0015         &      0.0007         &      0.0001         &     -0.0012         &     -0.0000         &     -0.0003         \\
Gender Gap in \%    &       -11.3         &         3.8         &         0.5         &       -10.0         &        -0.4         &       -18.3         \\
Observations        &       60615         &       60615         &       60615         &       60615         &       60615         &       58259         \\
\hline\hline \multicolumn{7}{p{\linewidth}}{\footnotesize \textit{Notes}: Standard errors in parentheses. *p$<$ 0.10, **p$<$ 0.05, ***p$<$ 0.001.}\\ \end{tabular}}


==> Tables/top_a6_table.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\hline\hline
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
                    &\multicolumn{1}{c}{Interview Promotion}&\multicolumn{1}{c}{Hired Promotion}\\
\hline
main                &                     &                     \\
Female              &       1.501\sym{***}&       1.425\sym{*}  \\
                    &     (0.541)         &     (0.772)         \\
\hline
Outcome Mean        &      0.4815         &      0.1650         \\
Av ME for Women     &      0.2722         &      0.1758         \\
Gender Gap in \%    &        56.5         &       106.5         \\
LR chi2             &         297         &         232         \\
\hline\hline \multicolumn{3}{p{\linewidth}}{\footnotesize \textit{Notes}: Standard errors in parentheses. *p$<$ 0.10, **p$<$ 0.05, ***p$<$ 0.001.}\\ \end{tabular}}

